Search for the associated production of the Higgs boson with a top quark pair in multilepton final states with the ATLAS detector

A search for the associated production of the Higgs boson with a top quark pair is performed in multilepton final states using 20.3 fb$^{-1}$ of proton-proton collision data recorded by the ATLAS experiment at $\sqrt{s}=8$ TeV at the Large Hadron Collider. Five final states, targeting the decays $H\to WW^*$, $\tau\tau$, and $ZZ^*$, are examined for the presence of the Standard Model (SM) Higgs boson: two same-charge light leptons ($e$ or $\mu$) without a hadronically decaying $\tau$ lepton; three light leptons; two same-charge light leptons with a hadronically decaying $\tau$ lepton; four light leptons; and one light lepton and two hadronically decaying $\tau$ leptons. No significant excess of events is observed above the background expectation. The best fit for the $t\bar t H$ production cross section, assuming a Higgs boson mass of 125 GeV, is $2.1 ^{+1.4}_{-1.2}$ times the SM expectation, and the observed (expected) upper limit at the 95% confidence level is 4.7 (2.4) times the SM rate. The $p$-value for compatibility with the background-only hypothesis is $1.8\sigma$; the expectation in the presence of a Standard Model signal is $0.9\sigma$.

==> SelectionTable.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
  \begin{center}
    {\small     
    \begin{tabular}{|c|c|c|c|c|c|c|}
      \hline
   %                        &  \bf{Leptons}  & \multicolumn{2}{c|}{ \bf{Selection} } &  \bf{Jets} &  \bf{B-Tags} &  \bf{Hadronic Taus} \\
                           & \multicolumn{3}{c|}{ \bf{Leptons} } &  \bf{Jets} &  \bf{B-Tags} &  \bf{Hadronic Taus} \\
 \hline
\multirow{2}{*}{\bf{Common}}    &  & \multicolumn{2}{c|}{$p_{T}>10$~GeV}                    & \multirow{2}{*}{$N_{j}\geq 2$} & \multirow{2}{*}{$N_{b}\geq1$} & \multirow{2}{*}{$p_{T}^{\tau} >$ 25~GeV} \\
                                &  & \multicolumn{2}{c|}{$\geq$ 1 trigger matched lepton}  &                          &                          &                                        \\
      \hline
 \multirow{11}{*}{\bf{2l}}    &   \multirow{11}{*}{$N_{l}=2$}  
                                   & \multicolumn{2}{c|}{$\Sigma$Q$_{lep} = \pm 2$}    &  & \multirow{11}{*}{$N_{b}\geq 1$} & \multirow{11}{*}{$N_{\tau}=0$} \\
                              &    & \multicolumn{2}{c|}{$|\eta_{electron}| < 1.37$}   &  &  &  \\
                              &    & \multicolumn{2}{c|}{$p_{T}^{lead} > 25$~GeV}   &  &  &  \\
                              &    & \multicolumn{2}{c|}{$p_{T}^{sub} > 20$~GeV}     &  &  &  \\
                             \cline{3-5}
                             &     & \bf{2lee4j} & 2 e$^{\pm}$ &   \multirow{3}{*}{$N_{j}=4$} &  &  \\\cline{3-4}
                             &     & \bf{2lem4j} & 1 e$^{\pm}$, 1 $\mu^{\pm}$ &    &  &  \\\cline{3-4}
                             &     & \bf{2lmm4j} & 2 $\mu^{\pm}$ &    &  &  \\\cline{3-5}
                             &     & \bf{2lee5j} &  2 e$^{\pm}$   &   \multirow{3}{*}{$N_{j} \geq 5$} &  &  \\\cline{3-4}
                             &     & \bf{2lem5j} & 1 e$^{\pm}$, 1 $\mu^{\pm}$  &   &  &  \\\cline{3-4}
                             &     & \bf{2lmm5j} &  2 $\mu^{\pm}$    &    &  &  \\\cline{3-4}
      \hline
      \multirow{3}{*}{\bf{ 3l} }     &   \multirow{3}{*}{$N_{l}=3$}  & \multicolumn{2}{c|}{$p_{T}^{same~sign~leptons} > 20$~GeV}   
                                   &\multicolumn{2}{c|}{$N_{j} \geq 4 $ \& $N_{b} \geq 1$}  & \multirow{3}{*}{- }   \\
                             &    & \multicolumn{2}{c|}{$\Sigma \text{Q}_{lep}$=$\pm 1$} & \multicolumn{2}{c|}{or}  &   \\
                             &    &  \multicolumn{2}{c|}{$|M_{ll}^{OS~SF} - M_{Z}| > 10$~GeV}        &  \multicolumn{2}{c|}{$N_{j}=3 $ \& $ N_{b} \geq  2$}  &  \\
      \hline
  \multirow{5}{*}{\bf{2ltau}}     &  \multirow{5}{*}{$N_{l}=2$}    &  \multicolumn{2}{c|}{$\Sigma \text{Q}_{lep} = \pm 2$}        
                                       &\multirow{5}{*}{$N_{j} \geq4 $}  & \multirow{5}{*}{$N_{b} \geq 1$} & \multirow{2}{*}{$N_{\tau}=1$} \\
                             &     &  \multicolumn{2}{c|}{$p_{T}^{lead}  > 25$~GeV}   &                 &  &  \\
                             &     &   \multicolumn{2}{c|}{$p_{T}^{sub} > 15$~GeV}     &                &   & \multirow{2}{*}{Q$_{\tau}$ = -Q$_{lep}$} \\
                             &     &  \multicolumn{2}{c|}{ $|M_{ll} - M_{Z}| > 10$~GeV}     &          &   &  \\
      \hline
      \multirow{2}{*}{\bf{1l2tau}}  & \multirow{2}{*}{$N_{l}=1$} &  \multicolumn{2}{c|}{\multirow{2}{*}{$p_{T}^{lepton} $ $>$ 25~GeV}}& \multirow{2}{*}{$N_{j} \geq 3$} & \multirow{2}{*}{$N_{b} \geq 1$} &  $N_{\tau}=2$ \\     
                                                 % & & \multicolumn{2}{c|}{$p_{T}^{lepton} $ $>$ 25~GeV} &              & & $\Sigma \text{Q}_{\tau}=0$   \\     
                                                  & &  \multicolumn{2}{c|}{}     &        & & $\Sigma \text{Q}_{\tau}=0$   \\     
      \hline
    \multirow{8}{*}{\bf{4l}}     &    \multirow{8}{*}{$N_{l}=4$}  & \multicolumn{2}{c|}{$\Sigma$Q$_{lep}$=0}        & \multirow{8}{*}{$N_{j} \geq 2$} & \multirow{8}{*}{$N_{b} \geq 1$} &  \multirow{8}{*}{-}\\
                             &     & \multicolumn{2}{c|}{$p_{T}^{lead} > 25$~GeV}                   &  &    &   \\
                             &     & \multicolumn{2}{c|}{$p_{T}^{sub} > 15$~GeV}                   &  &    &   \\
                             &     & \multicolumn{2}{c|}{$M_{ll}^{OS~SF} \geq 10$~GeV}                   &  &    &   \\
                             &     &\multicolumn{2}{c|}{100~GeV $<$ $M_{4l} < 500$~GeV} &  &  &  \\
                             &     &\multicolumn{2}{c|}{$|M_{ll}^{OS~SF} - M_{Z}| > 10$~GeV} &  &  &  \\\cline{3-4}
                             &     &  \multirow{2}{*}{\bf{Z-depleted}} & 0 OS SF &  &  &  \\
                             &     &    & lepton pairs &  &  &  \\\cline{3-4}
                             &     & \multirow{2}{*}{\bf{Z-enriched}} & $\geq$1 OS SF &  &  &  \\
                             &     &  & lepton pairs &  &  &  \\
      \hline
    \end{tabular}
    }
    \caption{\label{Tab:SelectionsSummary} Summary of event selections for five analysis channels. The acronym ``OS SF" stands for an opposite sign same-flavour lepton pair. $M_{ll, OS-SF} $ is the invariant mass of two leptons with opposite charge sign and of the same-flavour.
    The b-jets are included in the total jet multiplicity count.}
  \end{center}
\end{table}


